On the effective magnetostrictive properties of anisotropic magneto-active elastomers in the small-deformation limit

Magneto-active elastomers (MAEs) are composite materials comprising an elastomer matrix with embedded magnetic particles, endowing the composite with coupled effective magneto-mechanical responses. It is widely reported that anisotropic MAEs exhibit much stronger magneto-mechanical coupling than isotropic MAEs. However, most efforts to model effective magneto-mechanical properties of MAEs via homogenization focused on isotropic microstructures or those with large separations between particles, to use analytical solutions. In this work, we introduce a periodic homogenization approach to compute effective magneto-mechanical properties of anisotropic MAEs, and analyze microstructural features that enhance the magneto-mechanical coupling. Using the finite element method, we numerically determine the effect of particle shape, gap, and voids on the effective stiffness, permeability, and magneto-mechanical coupling tensors for chain-like periodic microstructures. Using insights gained from the full-field simulations, we derive an analytical expression for the magneto-mechanical coupling in the chain direction, in terms of the volume fraction, gap size, and properties of the matrix and particles. Results show that the overall magnetostriction of anisotropic MAEs is most sensitive to the gap between particles and the waviness of the particle chains, with smaller gap sizes and straighter chains yielding higher overall magnetostriction. Simulations also show that while isotropic MAEs elongate in a uniform magnetic field, anisotropic MAEs contract with much larger strain amplitudes, a result of the attractive forces between particles being much stronger in anisotropic MAEs than in isotropic MAEs. Results provide fundamental insights into the mechanisms that govern magneto-mechanical coupling in anisotropic MAEs, and constitute a toolbox of homogenized MAE material properties.

==> methods.tex <==
\FloatBarrier


==> theory-detailed.tex <==
We first briefly the review the theory of deformable magnetic bodies and a method to determine the effective magnetomechanical properties of MAE under the assumption of small strains and moderate magnetic fields. Consider a deformable body occupying a region \(\Omega\) of \(N\)-dimensional space, and surrounded by vacuum occupying the domain \(\Omega' = \mathbb{R}^n\backslash \Omega\). In the reference (undeformed) configuration, the material body occupies a domain \(\Omega^r\) of \(\mathbb{R}^N\) while the surrounding region of vacuum is denoted \(\Omega^{r'} = \mathbb{R}^n\backslash \Omega\). We introduce a set of Cartesian coordinates
\begin{align}
	X_I&, & I=\;&1,\dots,N
	\intertext{that parameterizes \(\mathbb{R}^N\). Under the application of mechanical and magnetic loads, the body deforms into a `current' configuration, under the mapping}
	x_i =\;& \chi_i(X_1, \dots, X_N) & \forall X \in\;& \Omega^r\,.
	\intertext{The mapping \(\chi_i\) is one-to-one and invertible. We use minuscule subscripts to denote vector components in the current configuration and majuscule subscripts to denote vector components in the reference configuration. We define the deformation gradient tensor \(F_{iJ}\) as}
	F_{iJ} =\;& F_{i,J} = \frac{\partial x_i}{\partial X_J}\,.
	\intertext{and the displacements \(u_I\) and \(u_i\) as}
	u_I(X_1, \dots, X_N) =\;& \chi_i(X_1,\dots,X_N) - X_I \\
	u_i(x_1, \dots, x_N) =\;& x_i - \chi^{-1}_I(x_1, \dots, x_N)\,.
	\intertext{The deformations and displacements have a physical interpretation only within \(\Omega^r\), where they represent the displacement of each material point from the reference to the current configuration. Outside the material body, we define a smooth extension of \(\chi_i\), where we assume that the displacement at infinity is 0, i.e.:}
	\lim_{|X|\rightarrow\infty} {\chi_i(X_1, \dots, X_N)} =\;& 0\,,
\end{align}
and that the extension of \(\chi_i\) conforms with the deformation of the material body on \(\partial \Omega^r\).

\FloatBarrier
\subsection{Magnetic Problem}
The magnetic problem is governed by Maxwell's equations, which may be expressed in the current configuration as:
\begin{subequations} \label{eq:mag-prob-curr}
	\begin{align}
		\mathrm{div}\,B =\;& 0 & \forall x \in\;& \mathbb{R}^N \\
		\mathrm{curl}\,H =\;& J & \forall x \in\;& \mathbb{R}^N \\
		n\cdot \llbracket B \rrbracket =\;& 0 & \forall x \in\;& S \\
		n \times \llbracket H \rrbracket =\;& K & \forall x \in\; & S
		\intertext{where \(B\) is the \emph{magnetic flux density}, \(H\) is the \emph{magnetic field intensity}, \(J\) is the \emph{volumetric current density}, \(K\) is the \emph{surface current density}, and \(n\) is the normal vector to an arbitrary (deformed) interface. The operators \(\mathrm{div}\,(\cdot) = \partial(\cdot)_i/\partial x_i\) and \(\mathrm{curl}\,(\cdot)_i = \epsilon_{ijk} \partial (\cdot)_j/\partial x_k\) (starting with miniscules) are taken with respect the coordinates \(x\) in the current configuration, and double brackets denote the ``jump'' operator: \(\llbracket(\cdot)\rrbracket = (\cdot)^e - (\cdot)^i\), where \((\cdot)^i\) and \((\cdot)^e\) are the values of a field on the interior and exterior sides of a boundary, respectively. Following the usual convention, we also define the \emph{magnetization}, \(M\), such that (using SI units):}
		B =\;& \mu_0 (H + M)
	\end{align}
\end{subequations}
Utilizing the transformation \(\chi\), the problem can be equivalently stated in the reference configuration:
\begin{subequations} \label{eq:mag-prob-ref}
	\begin{align}
		\mathrm{Div}\,B^r =\;& 0 & \forall X \in\;& \mathbb{R}^N \\
		\mathrm{Curl}\,H^r =\;& J^r & \forall X \in\;& \mathbb{R}^N \\
		n^r \cdot \llbracket B^r \rrbracket =\;& 0 & \forall X \in\;& S \\
		n^r \times \llbracket H^r \rrbracket =\;& K^r & \forall X \in\; & S\\
		B^r =\;& \mu_0 (H^r + M^r) & \forall X \in\;& \mathbb{R}^N \,,
	\end{align}
\end{subequations}
where the operators \(\mathrm{Div}\,(\cdot) = \partial(\cdot)_I/\partial X_I\) and \(\mathrm{Curl}\,(\cdot)_I = \epsilon_{IJK} \partial (\cdot)_J/\partial X_K\) (starting with majuscules) are taken with respect the coordinates \(X\) in the reference configuration, and all quantities with superscript ``\(r\)'' have been ``pulled back'' to the reference configuration. The current and reference magnetic fields are related by:
\begin{subequations} \label{eq:mag-prob-curr-to-ref}
	\begin{align}
		B^r_I =\;& (\mathrm{det}\,F) F^{-1}_{Ij} B_j \\
		H^r_I =\;& F^T_{Ij} H_j \\
		J^r_I =\;& (\mathrm{det}\,F) F^{-1}_{Ij} J_j \\
		K^r_I =\;& F^T_{Ij} K_j \\
		n^r_I\,\mathrm{d}A^r =\;& (\mathrm{det}\,F) F^T_{Ij} n_j\,\mathrm{d}A
	\end{align}
\end{subequations}

\FloatBarrier
\subsection{Mechanical Problem}
The mechanical problem is governed by the conservation of linear momentum, which is expressed in the current configuration as:
\begin{subequations} \label{eq:mech-prob-curr}
	\begin{align}
		\mathrm{div}\,\tau + f =\;& -t & \forall x \in\;& \Omega \label{eq:mech-prob-curr-cons-mom}\\
		n \cdot \llbracket \tau \rrbracket =\;& 0 & \forall x \in\;& \partial\Omega_N\, \label{eq:mech-prob-curr-trac-bc} \\
		u(x) =\;& \bar{u}(x) & \forall x \in\;& \partial\Omega_D\,,
	\end{align}
\end{subequations}
where \(\tau\) is the ``total'' stress that includes the Maxwell stress due to the magnetic field, \(f\) is the body force arising from all non-magnetic sources (\emph{e.g.}, gravity), \(t\) is a ``purely mechanical'' traction prescribed on a portion \(\partial \Omega_N\) of the boundary of the magnetoelasic solid, and \(\bar{u}\) is a displacement field prescribed on the complementary portion \(\partial \Omega_D = \partial\Omega \backslash \partial \Omega_N\) of the boundary. The form of the total stress and Maxwell stress is not unique; multiple equivalent definitions are possible, however, the particular form chosen will affect the form of the constitutive relation discussed in the following section.\citep{Bustamante2009a} For the purpose of this work, we adopt the following form for the Maxwell stress:
\begin{align} \label{eq:Maxwell-stress}
	\tau^M_{ij} =\;& B_i H_j - \frac{1}{2}H_k H_k \delta_{ij}\,.
	\intertext{We can then define the ``mechanical'' stress:}
	\sigma_{ij} =\;& \tau_{ij} - \tau^M_{ij} \,. \label{eq:stress-partition}
\end{align}
By definition, the mechanical stress is zero outside the magnetoelastic body: \(\sigma_{ij}=0 \; \forall x \in \Omega'\). Furthermore, Maxwell's equations~(\ref{eq:mag-prob-curr}) imply that the Maxwell stress is divergence-free outside the body: \(\mathrm{div}\,\tau^M=0 \; \forall x \in \Omega'\). This, combined with the absence of mechanical body forces \(f\) outside the body, implies that Equation~(\ref{eq:mech-prob-curr-cons-mom}) is automatically satisfied outside the body, and hence we have restricted the domain of Equation~(\ref{eq:mech-prob-curr-cons-mom}) to \(\Omega\).

We note that while the total stress \(\tau\) is symmetric, the Maxwell stress is not in general symmetric (in particular, it is asymmetric when the material is anisotropic and the magnetic field intensity \(H\) is not aligned one of the principal axes of the material), and thus the mechanical stress \(\sigma\) is not in general symmetric. This is a consequence of the body couple that arises when the applied magnetic field \(H\) and the magnetization \(M\) are non-parallel. However, due to the symmetry of the total stress, the conservation of angular momentum is implied. Using Equation~(\ref{eq:stress-partition}), it is possible to reformulate the problem with the introduction of a magnetic body force, \(f^M\):
\begin{subequations} \label{eq:mech-prob-curr-mech-form}
	\begin{align}
		\mathrm{div}\,\sigma + f^M + f =\;& 0 & \forall x \in\;& \Omega \,,
		\intertext{where \(f^M=\mathrm{div}\,\tau^M\). Due to the jump in the tangential (normal) components of \(B\) (\(H\)) at the material-vacuum interface, it is also necessary to account for a ``magnetic traction'' \(t^M\) on \(\partial \Omega_N\), necessitating a change in the boundary condition (\ref{eq:mech-prob-curr-trac-bc}), to:}
		n \cdot \sigma =\;& t + t^M & \forall x \in\;& \partial\Omega_N\,
	\end{align}
\end{subequations}
where \(t^M_i = n_j \llbracket \tau^M_{ji} \rrbracket \). However, due to the presence of body forces and surface tractions in Equation~(\ref{eq:mech-prob-curr-mech-form}), we find it more convenient to use the total-stress formulation (Equation~(\ref{eq:mech-prob-curr})) in the homogenization approach utilized in this paper.

As in the magnetic problem, it is possible to recast the mechanical problem in terms of the reference coordinates:
\begin{subequations} \label{eq:mech-prob-ref}
	\begin{align}
		\mathrm{Div}\,T =\;& 0 & \forall X \in\;& \Omega^r \\
		n^r \cdot \llbracket T \rrbracket =\;& t^r & \forall X \in\;& \partial \Omega^r_N \\
		u(x) =\;& \bar{u}(x) & \forall X \in\;& \partial \Omega^r_D\,,
	\end{align}
\end{subequations}
where \(T_{Ik} = (\mathrm{det}\,F) F^{-1}_{Ij} \tau_{jk}\) is the ``total first Piola-Kirchoff stress,'' \emph{i.e.} a total (mechanical plus Maxwell) traction in the current configuration referred to an undeformed area element in the reference configuration, and \(t^r\) is a traction referred to an area element reference configuration, such that \(t^r\,\mathrm{d}A^r = t\,\mathrm{d}A\).

\FloatBarrier
\subsection{Constitutive Behavior}
To complete the formulation of the problem, Equations~(\ref{eq:mag-prob-curr}) and~(\ref{eq:mech-prob-curr}) (or~(\ref{eq:mag-prob-ref}) and~(\ref{eq:mech-prob-ref})) must be augmented with constitutive laws. In general, such a constitutive law may be fully coupled, i.e. the magnetic quantities \(B\), \(H\), and \(M\) depend on each other as well as the mechanical quantities \(F\) and \(\tau\), and vice versa. The constitutive behavior can be expressed in terms of a free-energy function \(W\) which depends on one of the mechanical quantities and one of the magnetic quantities. Which of the quantities is chosen is arbitrary; however, the free-energies depending on different quantities can be related to each other by means of partial Legendre transforms. \citep{Bustamante2009a} For the purpose of this work, we consider a free-energy function expressed on a per-unit-mass basis in terms of the deformation gradient \(F\) and the magnetic field intensity \(H\):
\begin{align}
	W =\;& W(F, H) \,.
	\intertext{From this free energy the constitutive relations can be determined:}
	\sigma_{ij} =\;& \rho F_{ik} \frac{\partial W}{\partial F_{jk}} \label{eq:const-eqn-mech} \\
	M_i =\;& -\rho \frac{\partial W}{\partial H_i} \,. \label{eq:const-eqn-mag}
\end{align}
